Kit-Net: Self-Supervised Learning to Kit Novel 3D Objects into Novel 3D Cavities

In industrial part kitting, 3D objects are inserted into cavities for transportation or subsequent assembly. Kitting is a critical step as it can decrease downstream processing and handling times and enable lower storage and shipping costs. We present Kit-Net, a framework for kitting previously unseen 3D objects into cavities given depth images of both the target cavity and an object held by a gripper in an unknown initial orientation. Kit-Net uses self-supervised deep learning and data augmentation to train a convolutional neural network (CNN) to robustly estimate 3D rotations between objects and matching concave or convex cavities using a large training dataset of simulated depth images pairs. Kit-Net then uses the trained CNN to implement a controller to orient and position novel objects for insertion into novel prismatic and conformal 3D cavities. Experiments in simulation suggest that Kit-Net can orient objects to have a 98.9% average intersection volume between the object mesh and that of the target cavity. Physical experiments with industrial objects succeed in 18% of trials using a baseline method and in 63% of trials with Kit-Net. Video, code, and data are available at https://github.com/BerkeleyAutomation/Kit-Net.

==> includes/fig-reorienting-with-kit-net.tex <==
\begin{figure}
  \centering
  \includegraphics[width=0.48\textwidth]{figures/Orientation.PNG}
  \caption{\AB{this figure needs some labels, eg. $I^s$, $\hat{I}^g$, $I^g$}\textbf{Reorienting Objects with Kit-Net: }Kit-Net aligns objects from $I^s$ (left) to $\hat{I}^g$ (middle) given both positive (top right) and negative (bottom right) goal images $I^g$ by estimating ${_s}\hat{t}^g \in SE(3)$. Positive goal images are generated as described in Section~\ref{subsubsec:real-positive} while negative goal images are generated as described in Section~\ref{subsubsec:real-negative}.}
  \label{fig:Kit-Net-to-cavity}
\end{figure}
